Strongly Normalizing Audited Computation

Auditing is an increasingly important operation for computer programming, for example in security (e.g. to enable history-based access control) and to enable reproducibility and accountability (e.g. provenance in scientific programming). Most proposed auditing techniques are ad hoc or treat auditing as a second-class, extralinguistic operation; logical or semantic foundations for auditing are not yet well-established. Justification Logic (JL) offers one such foundation; Bavera and Bonelli introduced a computational interpretation of JL called $\lambda^h$ that supports auditing. However, $\lambda^h$ is technically complex and strong normalization was only established for special cases. In addition, we show that the equational theory of $\lambda^h$ is inconsistent. We introduce a new calculus $\lambda^{hc}$ that is simpler than $\lambda^h$, consistent, and strongly normalizing. Our proof of strong normalization is formalized in Nominal Isabelle.

==> abstract.tex <==
Auditing is an increasingly important operation for computer
programming, for example in security (e.g. to enable history-based
acce ss control) and to enable reproducibility and accountability
(e.g.  provenance in scientific programming).  Most proposed auditing
techniques are ad hoc or treat auditing as a second-class,
extralinguistic operation; logical or semantic foundations for
auditing are not yet well-established. Justification Logic (JL) offers
one such foundation; Bavera and Bonelli introduced a computational
interpretation of JL called JLh that supports auditing. However,
JLh is technically complex and strong normalization was only
established for special cases.  In addition, we show that the
equational theory of JLh is inconsistent.  We introduce a new
calculus JLhc that is simpler than JLh, consistent, and
strongly normalizing.  Our proof of strong normalization is formalized
in Nominal Isabelle.

